Interpolating Classifiers Make Few Mistakes

This paper provides elementary analyses of the regret and generalization of minimum-norm interpolating classifiers (MNIC). The MNIC is the function of smallest Reproducing Kernel Hilbert Space norm that perfectly interpolates a label pattern on a finite data set. We derive a mistake bound for MNIC and a regularized variant that holds for all data sets. This bound follows from elementary properties of matrix inverses. Under the assumption that the data is independently and identically distributed, the mistake bound implies that MNIC generalizes at a rate proportional to the norm of the interpolating solution and inversely proportional to the number of data points. This rate matches similar rates derived for margin classifiers and perceptrons. We derive several plausible generative models where the norm of the interpolating classifier is bounded or grows at a rate sublinear in $n$. We also show that as long as the population class conditional distributions are sufficiently separable in total variation, then MNIC generalizes with a fast rate.

==> qr-connections.tex <==
Consider the iterative algorithm defined by equation 1.8:
\begin{equation}\label{algorithm:qr}
	\beta_{k+1} = \beta_k + \frac{y-	\hat{f}_{D_{i-1}}(x_i) }{s_i^2} \Pi_{i-1}^{\perp} \phi_{x_i}
\end{equation}

We now show that this algorithm can be computed by a QR decomposition. We also show how with nothing but a QR decomposition, we can compute the average of the vectors $\beta_k$. We also show how to kernelize this calculation by leveraging a Cholesky decomposition of the empirical kernel matrix.


\begin{proposition}\label{prop:qr}
	Suppose $\phi$ maps into a $d$ dimensional space. Define the $d\times n$ dimensional matrix $\Phi$ to have $i$th column equal to $\phi_{x_i}$. Let $\Phi = QR$ be a QR decomposition of $\Phi$ and denote the $i$th column of $Q$ by $q_i$. Let $z=R^{-T} y$. Then $\beta_k = \sum_{i=1}^k q_{ i} z_i$.
\end{proposition}

\begin{proof}
First note that by construction, 
$$
	\phi_{x_k} = \sum_{i=1}^{k} R_{ik} q_i\,.
$$
Hence, 
$$
	 \Pi_{k-1}^{\perp} \phi_{x_k} = R_{kk} q_k\,.
$$
From this same calculation, we have that $s_k = R_{kk}$.


Consider the vector $z=R^{-T} y$. We have
$$
	z_k = \frac{y_k - \sum_{i=1}^{k-1} R_{ik} z_i}{R_{kk}}\,.
$$

Now let us proceed by induction. Certainly, for the base case, we have 
$$
\beta_1 = \frac{y_1}{s_i^2}  \phi_{x_i}=  \tfrac{y_1}{R_{11}^2} R_{11} q_1 = z_1 q_1\,.
$$ 

Now, suppose the formula holds for $i<k$ and consider 
$$
\begin{aligned}
\hat{f}_{D_{k-1}}(x_k) &= \langle \phi_{x_k} , \beta_{k-1} \rangle\\
&= \left\langle \sum_{j=1}^k  R_{jk} q_j, \sum_{\ell=1}^{k-1} q_\ell z_\ell \right\rangle\\
&= \sum_{j=1}^{k-1} R_{jk} z_j\,.
\end{aligned}
$$
Thus, 
$$
	z_k = \frac{y_k -\hat{f}_{D_{k-1}}(x_k) }{s_k}\,.
$$
and we have
$$
\beta_{k+1}-\beta_k = \frac{y_k -\hat{f}_{D_{k-1}}(x_k) }{s_k^2} \Pi_{k-1}^{\perp} \phi_{x_k} = z_k q_k\,,
$$
which completes the proof.
\end{proof}

Proposition~\ref{prop:qr} also allows us to compute the average of $\beta_i$ from the QR decomposition. Let $D$ denote the diagonal matrix with $k$th diagonal entry $1-\tfrac{k-1}{n}$. Then Proposition~\ref{prop:qr}{ immediately implies that 
\begin{equation}
	\frac{1}{n} \sum_{i=1}^n \beta_i = Q D R^{-T} y\,.
\end{equation}
This implies that computing the average of $\beta$ merely requires only $n$ floating point operations more than solving for the least-norm solution of $\Phi \beta =y$.

We can also kernelize the computation of the average. With slight abuse of notation, we can still let $\Phi$ denote the semiinfinite dimensional data matrix consisting of concatenation of $\phi_{x_i}$. This $\Phi$ will have a QR decomposition.  The kernel matrix $K = \Phi^T \Phi$ will have Cholesky decomposition $R^T R$ where $R$ is the same matrix as in the QR decomposition of $\Phi$. Our goal is to write $\beta_k$ as $\sum_{i=1}^n c_i \phi_{x_i}$. Let $P_k$ denote the diagonal matrix that projects onto the first $k$ standard coordinates in $\R^n$. Then we have $\beta_k = Q P_k z$ and
$$
	Kc = \Phi^T Q P_k z = R^T P_k z\,.
$$
Hence, $\beta_k = \Phi c$ with $c=R^{-1} P_k R^{-T} y$ and
$$
	\frac{1}{n} \sum_{i=1}^k \beta_k = R^{-1} D R^{-T} y\,.
$$

==> regret.tex <==



The paper is organized as follows. Section~\ref{sec:online-analysis} and \ref{sec:QR} will devote to answer the first question and provide a regret bound under essentially no assumptions. Section~\ref{sec:norm-growth} and \ref{sec:general-mixture} identify a host of scenarios under the i.i.d. assumption where the second question is answered, where notions of separation (on the data distribution) paint the common theme.


\section{No Assumption Analysis for Interpolation}
\label{sec:online-analysis}


\subsection{Notations}

Let us fix the notations first.

\begin{center}
\begin{tabular}{ c | c }
 Notations & Meaning \\ [0.5ex] 
 \hline \\
 $z_i = (x_i, y_i)$ & $i$-th data pair with input $x_i \in \cX \subset \Reals^d$ and label $y_i \in \cY \subset \Reals$\\
 $\phi_{x}$ & feature embedding $x \mapsto \phi_{x}$, $\Reals^d \rightarrow \Reals^p$ \\
 $K(x, x') = \langle  \phi_{x}, \phi_{x'} \rangle$ & kernel function $\cX \times \cX \rightarrow \Reals$ \\
 $\|f\|_{K}$ & RKHS norm of function $f$ with the corresponding kernel $K$\\
 $\Pi_{i}$ & projection operator to the ${\rm span}(\phi_{x_1}, \ldots, \phi_{x_{i}})$\\
 $D_i =\{ (x_j, y_j) \}_{j=1}^{i}$ & dataset at index $i$ \\
 $s_i$ & Euclidean distance of $\phi_{x_i}$ to the ${\rm span}(\phi_{x_1}, \ldots, \phi_{x_{i-1}})$ \\
 $s_{D_n\backslash i}$ & Euclidean distance of $\phi_{x_i}$ to the ${\rm span}(\phi_{x_1}, \ldots, \phi_{x_{i-1}}, \phi_{x_{i+1}}, \ldots, \phi_{x_n})$  \\
 $X_i \in \Reals^{i \times d}$& data matrix of $[x_1, \ldots, x_i ]^\top$ \\
 $X_{D_n \backslash i} \in \Reals^{(n-1) \times d}$ & data matrix of $[x_1, \ldots, x_{i-1}, x_{i+1}, \ldots, x_n ]^\top$\\
 $K(X_i, X_j) \in \Reals^{i \times j}$ & kernel matrix on data \\
 $Y_i \circ X_i \in \Reals^{i \times d}$ & data matrix of $[y_1 x_1, \ldots, y_i x_i ]^\top$  \\
 $\widehat{f}_{D_{i}}$ & min-norm interpolator using dataset $D_i$ \\ [0.5ex] 
 \hline
\end{tabular}
\end{center}





We have the following equality holds. 
\begin{lemma}[norm growth]
	\label{lem:norm-growth}
	If the minimum norm interpolators $\widehat{f}_{D_{i}}$, $\widehat{f}_{D_{i-1}}$ are well-defined, then
	\begin{align}
		\big\| \widehat{f}_{D_{i}} \big\|_K^2 - \big\| \widehat{f}_{D_{i-1}}  \big\|_K^2 = s_i^{-2} \cdot \big( y_i -   \widehat{f}_{D_{i-1}}(x_i) \big)^2 \enspace.
	\end{align}
\end{lemma}


\subsection{Algebraic Proof}
\begin{proof}[Proof of Lemma~\ref{lem:norm-growth}]
	We will present a two-line algebraic proof. Define $\Phi_{i} \in \Reals^{i \times p}$ as the embedded feature matrix. 
	\begin{align}
		& \| \widehat f_{D_i} \|_K^2 = Y_i^\top [K(X_i,X_i)]^{-1} Y_i \\
		&= [y_i, Y_{i-1}^{\top}] 
		\left[
		\begin{matrix}
			s_i^{-2} & -s_i^{-2} K(x_i, X_{i-1}) [K(X_{i-1}, X_{i-1})]^{-1}  \\
			-s_i^{-2}  [K(X_{i-1}, X_{i-1})]^{-1} K(X_{i-1}, x_i) & [\Phi_{i-1} \Phi_{i-1}^\top - \Phi_{i-1} \phi_{x_i} \frac{1}{K(x_i, x_i)} \phi_{x_i}^{\top} \Phi_{i-1}^\top   ]^{-1} 
		\end{matrix}
		\right]
		\left[
		\begin{matrix}
			y_i \\
			Y_{i-1}
		\end{matrix}
		\right] \\
		& =  s_i^{-2} \big[ y_i^2 - 2 y_i \widehat f_{D_{i-1}}(x_i) + + \big(  \phi_{x_i}^{\top} \Phi_{i-1}^\top  [\Phi_{i-1}\Phi_{i-1}^\top]^{-1} Y_{i-1} \big)^2 \big] + Y_{i-1}^\top [K(X_{i-1},X_{i-1})]^{-1} Y_{i-1}
	\end{align}
	Observing that $ \phi_{x_i}^{\top} \Phi_{i-1}^\top  [\Phi_{i-1}\Phi_{i-1}^\top]^{-1} Y_{i-1} = \widehat f_{D_{i-1}}(x_i)$ completes the proof.
\end{proof}


\subsection{Geometric Proof}
In this section, we will sketch a geometric proof of the key Lemma (in the interpolation case without explicit regularization). The proof naturally gives rise to an online algorithm for solving min-norm interpolators.

\begin{proof}[Proof of Lemma~\ref{lem:norm-growth}]
	We give a simple geometric proof when $p$---the dimension of $\phi_x$---is finite, the infinite case can be extended accordingly.
	\begin{figure}[htbp]
		\centering
		\hspace{4cm}
		\includegraphics[width=0.6\linewidth]{graphics/geometric_proof.pdf}
		\caption{Illustration of the geometric proof.}
	\end{figure}
	
	Recall that $\widehat{f}_{D_i}(x)$ is a linear function in $\phi_x$
	\begin{align}
		\widehat{f}_{D_i}(x) = \langle \phi_x, \widehat{\beta}_{i} \rangle \enspace,
	\end{align}
	where $\widehat{\beta}_{i} \in \Reals^p$ lies in the ${\rm span}(\phi_{x_1}, \ldots, \phi_{x_{i}})$. Let us compare $\widehat \beta_i$ and $\widehat \beta_{i-1}$. Observe that one must have
	\begin{align}
		\Pi_{i-1} \widehat\beta_{i} = \widehat\beta_{i-1} \enspace.
	\end{align}
	This is because the function $g_1(x) := \langle \phi_x, \Pi_{i-1} \widehat\beta_{i}\rangle$ has to interpolate the dataset $D_{i-1}$ as $$g_1(x_j) \equiv \widehat{f}_{D_i}(x_j)$$ for $1\leq j \leq i-1$. On the span of $\Pi_{i-1}$, there is a unique interpolating solution to $D_{i-1}$, namely $\widehat\beta_{i-1}$, thus proving the observation. Therefore,
	\begin{align}
		\widehat \beta_i &= \widehat \beta_{i-1} + \Pi_{i-1}^{\perp} \widehat \beta_i  \\
		&=  \widehat \beta_{i-1} + c \cdot \Pi_{i-1}^{\perp} \phi_{x_i}
	\end{align}
	with some constant $c$
	since $\widehat \beta_i$ lies in the span of $\{\phi_{x_1}, \ldots, \phi_{x_{i-1}} \} \cup \{ \phi_{x_{i}} \}$. To evaluate $c$, let us apply the function to the data point $(x_i, y_i)$
	\begin{align}
		y_i = \widehat{f}_{D_i}(x_i) = \langle \phi_{x_i}, \widehat{\beta}_{i} \rangle &= \langle \phi_{x_i}, \widehat{\beta}_{i-1} \rangle + c \cdot \langle \phi_{x_i},  \Pi_{i-1}^{\perp} \phi_{x_i} \rangle\\
		&=\widehat{f}_{D_{i-1}}(x_i) + c \cdot s_i^2 \enspace.
	\end{align}
	Thus, we have proved
	\begin{align}
		\widehat \beta_i = \widehat \beta_{i-1} + \frac{y_i - \widehat{f}_{D_{i-1}}(x_i)}{s_i^2} \cdot \Pi_{i-1}^{\perp} \phi_{x_i} \enspace.
	\end{align}
	Evaluating the norm on both sides of the equation will conclude the proof.
\end{proof}

\subsection{An Online Interpolation Algorithm}
The first consequence from the geometric proof of Lemma~\ref{lem:norm-growth} is an online algorithm.

\medskip
\begin{algorithm}[h]
	\label{alg:online-alg}
 \KwData{A sequence of data $\{z_i\}_{i=1}^{n}$. A feature embedding $\phi:\Reals^d \rightarrow \Reals^p$ that corresponds to an RKHS.}
 \KwResult{A min-norm interpolation function $\widehat{f}_{D_{i-1}}: \cX \rightarrow \cY$ on all past data $D_{i-1}$ at each time stamp $i$.}
 Initialization: Set $\widehat \beta_1 = \mathbf{0} \in \Reals^p$ and $\widehat f_{\cD_1} = 0$, and $i=0$ \;
 \While{$i < n$}{
   Set $i = i+1$ \;
   Receive a new data $z_i = (x_i, y_i)$ \;
   Make prediction based on the previous interpolator $\widehat f_{D_{i-1}}$ and record the error $e_i = y_i - f_{D_{i-1}}(x_i)$ \;
   Update the vector $\widehat \beta_i$
   $$
   \widehat \beta_i = \widehat \beta_{i-1} + \frac{e_i}{\| \Pi_{i-1}^{\perp} \phi_{x_i} \|^2} \cdot \Pi_{i-1}^{\perp} \phi_{x_i} \enspace,
   $$
   and the corresponding min-norm interpolation function $\widehat{f}_{D_{i}}(x) = \langle \phi_x,  \widehat \beta_i \rangle$ \;
 }
 \caption{Online Min-norm Interpolation Algorithm.}
\end{algorithm}
\medskip

Note that the function update can be written equivalently in the kernel form: define $g_i(x)$
\begin{align}
	g_i(x) = K(x, x_i) -  K(x, X_{i-1}) [K(X_{i-1}, X_{i-1}) ]^{-1} K(X_{i-1}, x_i) 
\end{align}
then
\begin{align}
	\widehat{f}_{D_{i}}(x) = \widehat{f}_{D_{i-1}}(x) + \frac{e_i}{g_i(x_i)}  g_i(x) \enspace.
\end{align}
\tl{Ben will connect to online QR as he sees fit.}



\paragraph{Regret Bound}
The second consequence from Lemma~\ref{lem:norm-growth} is a regret bound.
\begin{theorem}[Regret bound]
	\label{thm:regret}
	Assume 
	\begin{align}
		s_i^2 \leq &\sup_{1\leq i\leq n} K(x_i, x_i) \leq K_1 \enspace, ~~\text{and}\\
		s_{D_n\backslash i}^2 \geq &\inf_{1\leq i \leq n} K(x_i, x_i) - K(x_i, X_{D_n \backslash i})[K(X_{D_n \backslash i}, X_{D_n \backslash i})]^{-1} K(X_{D_n \backslash i}, x_i) \geq K_0 \enspace.
	\end{align}
	Then the Online Interpolation Algorithm~\ref{alg:online-alg} satisfies the following regret bound
	\begin{align}
		K_0 \cdot \frac{\| \widehat f_{D_n} \|_{K}^2}{n} \leq \frac{1}{n}\sum_{i=1}^{n} \big(y_i - \widehat{f}_{D_{i-1}} (x_i) \big)^2 \leq K_1 \cdot \frac{\| \widehat f_{D_n} \|_{K}^2}{n} \enspace,
	\end{align}
	where $\widehat{f}_{D_{i-1}}$ is the min-norm interpolator on the past data $D_{i-1}$. In the binary classification setting with $\cY = \{\pm 1\}$, we further have
	\begin{align}
		\frac{1}{n}\sum_{i=1}^{n} \mathbbm{1}_{y_i \widehat{f}_{D_{i-1}} (x_i) \leq 0 } \leq K_1 \cdot \frac{\| \widehat f_{D_n} \|_{K}^2}{n} \enspace.
	\end{align}
\end{theorem}

\begin{corollary}[Polyak-Averages]
	Define the Polyak average of interpolators
	$$
	\widehat f_n = \frac{1}{n} \sum_{i=1}^{n} \widehat f_{D_i}
	$$
	then the following out-of-sample error holds,
	\begin{align}
		\mathbb{E} \left[ \mathbbm{1}_{ \by \widehat f_n (\bx) } \right] \leq K_1 \cdot \frac{ \E \big[ \| \widehat f_{D_n} \|_K^2 \big]}{n} \enspace.
	\end{align}
\end{corollary}
	
